Simulating photonic devices with noisy optical elements

Quantum computers are inherently affected by noise. While in the long-term error correction codes will account for noise at the cost of increasing physical qubits, in the near-term the performance of any quantum algorithm should be tested and simulated in the presence of noise. As noise acts on the hardware, the classical simulation of a quantum algorithm should not be agnostic on the platform used for the computation. In this work, we apply the recently proposed noisy gates approach to efficiently simulate noisy optical circuits described in the dual rail framework. The evolution of the state vector is simulated directly, without requiring the mapping to the density matrix framework. Notably, we test the method on both the gate-based and measurement-based quantum computing models, showing that the approach is very versatile. We also evaluate the performance of a photonic variational quantum algorithm to solve the MAX-2-CUT problem. In particular we design and simulate an ansatz which is resilient to photon losses up to $p \sim 10^{-3}$ making it relevant for near term applications.

==> appendices/circ_visualization.tex <==
In this appendix we display the circuits that we implement for the simulations in Section \ref{tests}. The translations from circuit defined in Qiskit \cite{qiskit} to optical circuit are performed with the QiskitConverter functionality of Perceval \cite{Perceval}.
\begin{figure*}[htp]
\centering
\begin{minipage}{0.25\textwidth}
\includegraphics[width=\textwidth]{plots/X_gate_qiskit.pdf}
\end{minipage}
\begin{minipage}{0.40\textwidth}
\includegraphics[width=\textwidth]{plots/X_circuit.pdf}
\end{minipage}
\caption{On the left the circuit for the X gate in GBQC. On the right the corresponding optical circuit.}
\label{X_circuits}
\end{figure*}

\begin{figure*}[htp]
\centering
\begin{minipage}{0.25\textwidth}
\includegraphics[width=\textwidth]{plots/Bell_state_qiskit.pdf}
\end{minipage}
\begin{minipage}{\textwidth}
\includegraphics[width=\textwidth]{plots/Bell_circuit}
\end{minipage}
\caption{On the top the circuit for the Bell state in GBQC. On the bottom the corresponding optical circuit.}
\label{Bell_circuits}
\end{figure*}

\begin{figure*}[htp]
\centering
\begin{minipage}{0.25\textwidth}
\includegraphics[width=\textwidth]{plots/MBQC_X_gate_qiskit.pdf}
\end{minipage}
\begin{minipage}{\textwidth}
\includegraphics[width=\textwidth]{plots/MBQC_X_circuit.pdf}
\end{minipage}
\caption{On the top the circuit required to prepare the cluster state for the X gate in MBQC. On the bottom the corresponding optical circuit. Measurements for the MBQC are not shown.}
\label{MBQC_X_circuits}
\end{figure*}

\begin{figure*}[htp]
\centering
\begin{minipage}{\textwidth}
\includegraphics[width=\textwidth]{plots/VQA.pdf}
\end{minipage}
\caption{Optical circuit ansatz for the VQA solving the max 2-cut on a square graph.}
\label{VQA_ansatz}
\end{figure*}

